Fusion of Radio and Camera Sensor Data for Accurate Indoor Positioning

Indoor positioning systems have received a lot of attention recently due to their importance for many location-based services, e.g. indoor navigation and smart buildings. Lightweight solutions based on WiFi and inertial sensing have gained popularity, but are not fit for demanding applications, such as expert museum guides and industrial settings, which typically require sub-meter location information. In this paper, we propose a novel positioning system, RAVEL (Radio And Vision Enhanced Localization), which fuses anonymous visual detections captured by widely available camera infrastructure, with radio readings (e.g. WiFi radio data). Although visual trackers can provide excellent positioning accuracy, they are plagued by issues such as occlusions and people entering/exiting the scene, preventing their use as a robust tracking solution. By incorporating radio measurements, visually ambiguous or missing data can be resolved through multi-hypothesis tracking. We evaluate our system in a complex museum environment with dim lighting and multiple people moving around in a space cluttered with exhibit stands. Our experiments show that although the WiFi measurements are not by themselves sufficiently accurate, when they are fused with camera data, they become a catalyst for pulling together ambiguous, fragmented, and anonymous visual tracklets into accurate and continuous paths, yielding typical errors below 1 meter.

==> discussion.tex <==
\section{Discussion}

As mentioned in the introduction, the key aim of this work is to present a generic radio+vision tracking framework that is applicable to many different scenarios. In general, these can be divided into two broad classes: receiver-centric (as shown in the evaluation) and transmitter-centric.

\noindent{\textbf{Receiver-centric:}} In receiver-centric applications, the mobile device receives RSSI measurements from multiple basestations or access points. In addition, the tracklets need to be sent to the mobile device as well. Computation of the position of the device is undertaken locally, for instance, on a user's smartphone. Typically, in this class of application, the key focus is on preserving the user's privacy. Users should not have to share private data generated by their mobile devices with a central infrastructure, but only exploit it locally to position themselves. By the same token, raw video footage should not be communicated to individuals, without appropriate pre-processing to remove sensitive information that reveal the identities of people and objects moving in the environment. A challenge is how to prevent privacy leaks through inadvertent radio emissions, which would allow a third party (e.g. a supermarket operator or airport personnel) to match a user's visual trajectory to a particular mobile device. The ideal situation is to never send any radio signals but yet still obtain all necessary measurements. When using WiFi, signal strengths can be obtained by passively scanning for APs, i.e. to never send active probe requests. To obtain the tracklets without associating to an AP is a greater challenge, but this can be accomplished using beacon stuffing. In this setup, WiFi-enabled cameras can disseminate anonymous tracklets as part of their periodic beacon transmissions. It must be noted however that a malicious attacker can exploit techniques presented in this paper (vision + RF) to track a user with high precision if the user is creating any form of identifiable RF emission (e.g. cellular beacons). To overcome a determined attacker, techniques need to be put into place to randomize and encrypt MAC addresses and jitter signal strength emissions.

\noindent{\textbf{Transmitter-centric:}} This class of applications typically is encountered in commercial, industrial and enterprise settings, where the position of many objects needs to be determined in a cost effective manner and where the infrastructure and objects are controlled by a single entity. Low-cost tags (e.g. iBeacons/BTLE) can be affixed to parcels, vehicles and other objects and these periodically emit identifying beacons. The infrastructure receives these beacons and with the aid of the visual trajectory, calculates the position of the objects centrally. This in many ways is a simpler scenario as all the tracklets and radio measurements can be combined to enhance the performance of the multi-hypothesis tracker. Note that no modification is needed to the presented algorithm, it simply is implemented centrally for all devices, rather than distributed across each device.

